Direct Neural Machine Translation with Task-level Mixture of Experts models

Direct neural machine translation (direct NMT) is a type of NMT system that translates text between two non-English languages. Direct NMT systems often face limitations due to the scarcity of parallel data between non-English language pairs. Several approaches have been proposed to address this limitation, such as multilingual NMT and pivot NMT (translation between two languages via English). Task-level Mixture of expert models (Task-level MoE), an inference-efficient variation of Transformer-based models, has shown promising NMT performance for a large number of language pairs. In Task-level MoE, different language groups can use different routing strategies to optimize cross-lingual learning and inference speed. In this work, we examine Task-level MoE's applicability in direct NMT and propose a series of high-performing training and evaluation configurations, through which Task-level MoE-based direct NMT systems outperform bilingual and pivot-based models for a large number of low and high-resource direct pairs, and translation directions. Our Task-level MoE with 16 experts outperforms bilingual NMT, Pivot NMT models for 7 language pairs, while pivot-based models still performed better in 9 pairs and directions.

==> experts_plots.tex <==
\begin{figure*}[htb]
  \centering
  \subfloat[]{%
    \includegraphics[trim={1cm 0 0 0},clip,width=\textwidth]{figures/experts_plots/TaskMoE_16_C128_B256_all_4yy_2xx_dt_c/tl_mapping_a/ckpt-1m/enc_3_01010000_web1_1_.png}}\hfill \\
  \subfloat[]{%
    \includegraphics[trim={1cm 0 0 0 1cm},clip,scale=0.52,width=\textwidth]{figures/experts_plots/TaskMoE_16_C128_B256_all_4yy_2xx_dt_c/tl_mapping_a/ckpt-1m/dec_3_01010000_web1_1_.png}}\hfill
\caption{}
\label{}
\end{figure*}
\begin{comment}
  \subfloat[]{%
    \includegraphics[width=.33\textwidth]{figures/experts_plots/TaskMoE_16_C128_B256_all_4yy_2xx_dt_c/tl_mapping_a/ckpt-1m/dec_1_01010000_web1_1_.png}}\hfill
\subfloat[]{%
    \includegraphics[width=.33\textwidth]{figures/experts_plots/TaskMoE_16_C128_B256_all_4yy_2xx_dt_c/tl_mapping_a/ckpt-1m/dec_2_01010000_web1_1_.png}}\hfill
  \subfloat[]{%
    \includegraphics[width=.33\textwidth]{figures/experts_plots/TaskMoE_16_C128_B256_all_4yy_2xx_dt_c/tl_mapping_a/ckpt-1m/dec_3_01010000_web1_1_.png}}\hfill

\caption{}
\label{}
\end{comment}

